Zeroth-order Low-rank Hessian Estimation via Matrix Recovery

A zeroth-order Hessian estimator aims to recover the Hessian matrix of an objective function at any given point, using minimal finite-difference computations. This paper studies zeroth-order Hessian estimation for low-rank Hessians, from a matrix recovery perspective. Our challenge lies in the fact that traditional matrix recovery techniques are not directly suitable for our scenario. They either demand incoherence assumptions (or its variants), or require an impractical number of finite-difference computations in our setting. To overcome these hurdles, we employ zeroth-order Hessian estimations aligned with proper matrix measurements, and prove new recovery guarantees for these estimators. More specifically, we prove that for a Hessian matrix $H \in \mathbb{R}^{n \times n}$ of rank $r$, $ \mathcal{O}(nr^2 \log^2 n ) $ proper zeroth-order finite-difference computations ensures a highly probable exact recovery of $H$. Compared to existing methods, our method can greatly reduce the number of finite-difference computations, and does not require any incoherence assumptions.

==> tex/matrix-compressed-sensing.tex <==

% \section{Hessian Estimation Part II: Matrix Compressed Sensing} 

% \textcolor{red}{(double check the left coherence condition)} 

\begin{lemma}
    \label{lem:order} 
    Let $ \u, \v \overset{iid}{\sim} \mathrm{Unif} \( \mathbb{S}^{n-1} \) $. Then we have 
    \begin{align*} 
        \E \[ \( n \u_{:r} \u_{:r}^\top \)^p \otimes \( n \v \v^\top \)^p \] 
        \preceq 
        \frac{p!}{2} ( 6 n (r+2 ) )^{p-2} n ( r + 2 ) I_{n^2}
    \end{align*}
    and
    \begin{align*}
        \E \[ \( n \u \u^\top \)^p \otimes \( n \v_{:r} \v_{:r}^\top \)^p \] 
        \preceq 
        \frac{p!}{2} ( 6 n (r+2 ) )^{p-2} n ( r + 2 ) I_{n^2} , 
    \end{align*}  
    where $ \u_{:r} = \( u_1, u_2, \cdots, u_r, 0 , 0 , \cdots ,0 \)^\top $ and $ \v_{:r} = \( v_1, v_2, \cdots, v_r, 0 , 0 , \cdots ,0 \)^\top $. 
\end{lemma} 

\begin{proof} 
    We derive a Loewner upper bound for $ \E \[ \( n \u_{:r} \u_{:r}^\top \)^p \otimes \( n \v \v^\top \)^p \] $. The upper bound for $ \E \[ \( n \u \u^\top \)^p \otimes \( n \v_{:r} \v_{:r}^\top \)^p \] $ follows similarly. 
    We start with $ p =2$. 
    For this case, we have 
    \begin{align*} 
        n^2 \E \[ \( \v \v^\top \)^2 \] 
        = n I_n, 
    \end{align*} 
    and 
    \begin{align*}
        n^2 \E \[ \( \u_{:r} \u_{:r}^\top \)^2 \]
        = 
        n^2 \E \[ \( \sum_{i=1}^r u_i^2 \) \u_{:r} \u_{:r}^\top \] 
        \preceq 
        n^2 \( \frac{r-1}{n^2} + \frac{3}{n(n+2)} \) I_n 
        \preceq 
        (r+2) I_n . 
    \end{align*} 
    
    For $p > 2$, we have 
    \begin{align*} 
        n^p \E \[ \( \v \v^\top \)^p \] 
        = 
        n^p \E \[ \v \v^\top \] = n^{p-1} I_n, 
    \end{align*} 
    and 
    \begin{align*} 
        n^p \E \[ \( \u_{:r} \u_{:r}^\top \)^p \] 
        = 
        n^p \E \[ \| \u_{:r} \|^{2p-2} \u_{:r} \u_{:r}^\top \] 
        = 
        n^p \E \[ \( \sum_{i=1}^r u_i^2 \)^{p-1} \u_{:r} \u_{:r}^\top \] 
        \preceq 
        n^p \E \[ r^{p-1} \( \sum_{i=1}^r u_i^{2p} \) \u_{:r} \u_{:r}^\top \] 
    \end{align*} 
    where the last inequality uses Jensen's inequality. 

    \textcolor{red}{(check the exponent in the above equation.)}
    
    We apply Proposition \ref{prop:p} to the above inequality, and obtain 
    \begin{align*} 
        & \; n^p \E \[ \( \u_{:r} \u_{:r}^\top \)^p \] 
        \preceq 
        n^p r^{p-1} \( \frac{ (r-1) (2p)!! }{ n \cdot n (n+2) \cdots (n+2p-2) } + \frac{(2p+2)!!}{ n (n+2) \cdots (n+2p) } \) \\ 
        \preceq& \; 
        \frac{p!}{2} (6 (r + 2) )^{p-1} I_n . 
        % \preceq 
        % p! (r + 2)^{p}  I_n . 
    \end{align*} 

    By the calculus rule of Kronecker product, we have 
    \begin{align*} 
        \E \[ \( n \u_{:r} \u_{:r}^\top \)^p \otimes \( n \v \v^\top \)^p \] 
        \preceq 
        \frac{p!}{2} (6 (r + 2) )^{p-1} I_n \otimes \( n^{p-1} I_n \) , 
    \end{align*} 
    which concludes the proof since the Loewner upper bound for $ \E \[ \( n \u \u^\top \)^p \otimes \( n \v_{:r} \v_{:r}^\top \)^p \]  $ follows similarly. 
    % Therefore, 

\end{proof} 


\begin{lemma}
    \label{lem:concent}
    Consider the matrix compressed sensing estimator. 
    Let 
    \begin{align*}
        \mathcal{E}_3 := \left\{ \left\| \P_{T_r} \S \P_{T_r} - \P_{T_r} \right\| \le \frac{1}{4 \sqrt{r}} 
        \text{ and } 
        \left\| \S \P_{T_r} - \P_{T_r} \right\| \le \frac{1}{4 \sqrt{r}} 
        \text{ and } 
        \left\| \P_{T_r} \S - \P_{T_r} \right\| \le \frac{1}{4 \sqrt{r}} . 
        \right\}
    \end{align*} 
    % $  $. 
    Then there exists a constant $c$, such that for any $\delta \in (0,1)$ if $ M \ge c \cdot nr^{1.5} \log \( 1/\delta \) $, then $\Pr \( \mathcal{E}_3 \) \le 1 - \delta $. 
\end{lemma}

\begin{proof}

    By Lemma \ref{lem:order}, we have 
    \begin{align*} 
        \E \[ \( n \u_{:r} \u_{:r}^\top \otimes  n \v \v^\top \)^p \] 
        = 
        \E \[ \( n \u_{:r} \u_{:r}^\top \)^p \otimes \( n \v \v^\top \)^p \] 
        \preceq  
        \frac{p!}{2} ( 6 n (r+2 ) )^{p-2} n ( r + 2 ) I_{n^2}
        % ??????? 
    \end{align*} 
    
    % From here we can apply Lemma \ref{???}. 
    
    
    Since $H_r$ is symmetric and of rank $r$, there exists a basis $\mathcal{B}$ for $ \R^{n \times n} $ such that, in basis $ \mathcal{B} $, $P_{U_r} = I_n^{:r} := \begin{bmatrix} I_r & 0_{r \times (n-r)} \\ 0_{ (n-r) \times r} & 0_{ (n-r) \times (n-r)} \end{bmatrix}  $. Since the distribution of $\v$ and $\u$ are rotation-invariant and reflection-invariant, we know the distribution of $\v$ and $\u$ does not change after any change of basis. Therefore, we consider the random matrices $ \P_{T_r} \P_i \P_{T_r} $, $ \P_{T_r} \P_i $ and $ \P_i \P_{T_r} $ in basis $\mathcal{B}$. 
    
    % -------------------------------------------
    
    In basis $ \mathcal{B} $, we have, for any $p \ge 2$
    \begin{align} 
        \E \[ \( \P_{T_r} \P_i \P_{T_r} \)^p  \]
        \preceq  
        \E \[ \( n \( \u_{:r} \u_{:r}^\top \) \otimes \( n \v \v^\top \) \)^p  \] + \E \[ \( n \( \u \u^\top \) \otimes \( n \v_{:r} \v_{:r}^\top \) \)^p \] 
        \preceq 
        \frac{p!}{2} ( 12 n (r+2 ) )^{p-2} n ( r + 2 ) I_{n^2} , \label{eq:moment-bound}
    \end{align} 
    and thus 
    \begin{align*} 
        \E \[ \( \P_{T_r} \P_i \P_{T_r} - \P_{T_r} \)^p  \]  
        \preceq
        \frac{p!}{2} ( 24 n (r+2 ) )^{p-2} \cdot 4 n ( r + 2 ) I_{n^2}, \quad \forall p \ge 2. 
    \end{align*} 
    
    Since $ \E \[ \P_{T_r} \P_i \P_{T_r} \] = \P_{T_r} $ and $ \S = \frac{1}{M} \sum_{i=1}^M \P_{T_r} \P_i \P_{T_r} $, 
    we apply Theorem \ref{thm:zhu} to show that $ \left\| \P_{T_r} \S \P_{T_r} - \P_{T_r} \right\| \le \frac{1}{4 \sqrt{r}}  $ happens with high probability. Similarly, the Bernstein condition (\ref{eq:moment-bound}) holds for $ \P_{T_r} \P_i $ and $ \P_i \P_{T_r} $: 
    \begin{align*} 
        \E \[ \( \P_{T_r} \P_i \)^p  \] 
        \preceq 
        \frac{p!}{2} ( 12 n (r+2 ) )^{p-2} n ( r + 2 ) I_{n^2} 
        \quad \text{and} \quad 
        \E \[ \( \P_i \P_{T_r} \)^p  \] 
        \preceq 
        \frac{p!}{2} ( 12 n (r+2 ) )^{p-2} n ( r + 2 ) I_{n^2} , \;\; p \ge 2
    \end{align*} 
    Then two additional application of Theorem \ref{thm:mat-berstein} and a union bound conclude the proof. 
    
\end{proof}



\begin{lemma} 
    \label{lem:infeas-2} 
    Suppose $\mathcal{E}_3$ is true. Let $ \wh{H} $ be the solution of the constrained optimization problem, and let $\Delta := \wh{H} - H$. Then $ \| \P_{T_r} \Delta \|_2 \le 2n \| \P_{T_r}^\perp \Delta \|_2 $. 
\end{lemma} 

\begin{proof} 

    % Let $\mathc$
    
    % For the operator $\S : A \to LAR$, define $ \sqrt{\S} $ such that $ \sqrt{\S} : A \to \sqrt{L} A \sqrt{R} $. 
    Represent $\S$ as a matrix of size $ n^2 \times n^2 $. Let $ \sqrt{\S} $ be defined as a canonical matrix function. That is, $ \sqrt{\S} $ and $ \S $ share the same eigenvectors, and the eigenvalues of $ \sqrt{\S} $ are the square roots of the eigenvalues of $\S$. 
    Clearly, 
    \begin{align} 
        \| \sqrt{\S} \Delta \|_2 
        = 
        \| \sqrt{\S} \P_{T_r}^\perp \Delta + \sqrt{\S} \P_{T_r} \Delta \|_2 
        \ge 
        \| \sqrt{\S} \P_{T_r} \Delta \|_2 - \| \sqrt{\S} \P_{T_r}^\perp \Delta \|_2 . \label{eq:infeasible-2-3} 
    \end{align} 
    
    Clearly we have 
    \begin{align*} 
        \| \sqrt{ \S } \P_{T_r}^\perp \Delta \|_2 
        \le  
        n \| \P_{T_r}^\perp \Delta \|_2 . 
    \end{align*} 

    Also, by Lemma \ref{lem:concent}, we have 
    \begin{align} 
        & \; \| \sqrt{\S} \P_{T_r} \Delta \|_2^2 
        =  
        \< \sqrt{\S} \P_{T_r} \Delta, \sqrt{\S} \P_{T_r} \Delta \>
        = 
        \< \P_{T_r} \Delta, \P_{T_r} \S \P_{T_r} \Delta \> \nonumber \\ 
        =& \; 
        \| \P_{T_r} \Delta \|_2^2 - \< \P_{T_r} \Delta - \P_{T_r} \S \P_{T_r} \Delta , \P_{T_r} \Delta \> 
        \ge 
        \frac{1}{2} \| \P_{T_r} \Delta \|_2^2 . \label{eq:infeasible-2-4}
    \end{align} 

    % Therefore, we have $ \| \sqrt{\S} \P_{U_r} \Delta \|_2 \ge \frac{1}{2} \|  \Delta_{(1)} + \Delta_{(2)} \|_2 $. 
    % Suppose $ \Delta \neq 0 $. 
    % Then when $\mathcal{E}_1$ and $\mathcal{E}_2$ are true, (\ref{eq:infeasible}) gives 
    % Suppose, in order to get a contradiction, that $ \sqrt{\S} \Delta = 0 $ and $ \| \Delta_{(1)} + \Delta_{(2)} \|_2 > 10n^{2.5} \| \Delta_{(3)} + \Delta_{(4)} \|_2 $. 
    Since $ \wh{H} $ solves (\ref{eq:obj}), we know $ \S \Delta = 0 $, and thus $ \sqrt{\S} \Delta = 0 $. 
    Suppose, in order to get a contradiction, that $ \| \P_{T_r} \Delta \|_2 > 2n \| \P_{T_r}^\perp \Delta \|_2 $. 
    Then (\ref{eq:infeasible-2-3}) and (\ref{eq:infeasible-2-4}) yield  
    \begin{align*} 
        \| \sqrt{\S} \Delta \|_2 
        \ge 
        \frac{1}{2} \| \P_{T_r} \Delta \|_2 - n \| \P_{T_r}^\perp \Delta \|_2 > 0, 
    \end{align*} 
    which leads to a contraction. 
    % Finally, we have $ \sqrt{\S} \Delta = 0 $ if and only if $ \S \Delta = 0 $. 
    % This proves the first item. Similarly, we can prove the second and the third item. 

\end{proof}  

\begin{lemma}
    \label{lem:exist-cert-2}
    % Fix $\epsilon > 0$. 
    Define 
    \begin{align*}
        \mathcal{E}_4 := \left\{ \exists \; Y \in range(\S) : \| \P_{T_r} Y - \sign (H_r) \| \le \frac{1}{ n^{20} } 
        \quad \text{and} \quad 
        \| \P_{T_r}^\perp Y \| \le \frac{1}{2} \right\} . 
    \end{align*}
    Let $ m \ge c \cdot n r \log n $ for some constant $c$. Pick any $\delta \in (0,1)$. If $M = m L \ge c \cdot n r \log n \log (1/\delta)$ for some constant $c$, then $ \Pr \( \mathcal{E}_2 \) \ge 1 - \delta $. 
    % then with probability exceeding $1 - \frac{1}{n}$, 
    % Under event $\mathcal{E}_1 \cap \mathcal{E}_2 \cap \mathcal{E}_3 \cap \mathcal{E}_4 $, 
    % there exists $Y \in range(\S)$, such that 
    % \begin{align*} 
    %     \| \P_{T_r} Y - \sign (H_r) \| \le \frac{1}{ n^{20} } 
    %     \quad \text{and} \quad 
    %     \| \P_{T_r}^\perp Y \| \le \frac{1}{2} . 
    % \end{align*} 
    % Let $ \mathcal{E}_2 $
\end{lemma} 

% \textcolor{red}{(check this. this is off as well. )} 

\begin{proof} 
    Following \citep{gross2011recovering}, we define random projectors $ \wt{\S}_l $ ($1 \le l \le L$), such that 
    \begin{align*}
        \wt{\S}_l := \frac{1}{m} \sum_{j=1}^m \P_{m(l-1) + j} .  
    \end{align*}

    Then define 
    \begin{align*} 
        X_0 = \sign (H_r), \quad Y_i = \sum_{j=1}^i \wt{\S}_j \P_{T_r} X_{j-1}, \quad X_i = \sign (H_r) - \P_{T_r} Y_i , 
        \quad Z_i = \wt{\S}_i \P_{T_r} X_{i-1} , \quad \forall i \ge 1. 
    \end{align*} 
    
    From the above definition, we have 
    \begin{align*}  
        X_i = ( \P_{T_r} - \P_{T_r} \wt{\S}_i \P_{T_r} ) ( \P_{T_r} - \P_{T_r} \wt{\S}_{i-1} \P_{T_r} ) \cdots ( \P_{T_r} - \P_{T_r} \wt{\S}_1 \P_{T_r} ) X_0 . 
    \end{align*} 

    % Since $X_i \in T_r$ and $\wt{S}_{i+1}$ is independent of $X_i$, 
    We apply Lemma \ref{lem:concent} to $ \wt{\S}_1, \wt{\S}_2, \cdots , \wt{\S}_L $, and get 
    \begin{align}
        \| X_{L} \|_2 \le \frac{1}{4} \| X_{L} \|_2 \le \cdots \le \frac{1}{4^L} = \frac{1}{n^{20}} , 
        % \| X_{i+1} \|_2 \le \frac{1}{4} \| X_i \|_2 , 
        \label{eq:recur-2} 
    \end{align} 
    and 
    \begin{align*} 
        \| \P_{T_r} Y_{L} \|_2 \le \sum_{i=1}^L 
        \frac{1}{4} \| X_{i} \|_2 \le \frac{1}{2} . 
        % \cdots \le \frac{1}{4^L} = \frac{1}{n^{20}} 
    \end{align*} 
    
\end{proof}

\subsection{Proof of Theorem \ref{thm:main}}


\begin{proof}[Proof of Theorem \ref{thm:main}] 
    Let $\mathcal{E}_1$ and $\mathcal{E}_2$ be true. 
    Then there exists $Y$ such that $\< Y ,\Delta \> = 0$, since $\S \Delta = 0$. Thus we have
    \begin{align*}
        & \; \< \sign(H),  P_{U} \Delta P_{U} \> 
        = 
        \< \sign(H),  \Delta \> 
        = 
        \< \sign(H) - Y,  \Delta \>
        = 
        \< \P_T \( \sign(H) - Y \) ,  \Delta_T \> + \< \P_T^\perp \( \sign(H) - Y \) ,  \Delta_T^\perp \> \\ 
        =& \; 
        \< \sign(H) - \P_T Y ,  \Delta_T \> - \< \P_T^\perp  Y ,  \Delta_T^\perp \>
        \ge 
        - \frac{1}{n^{20}} \| \Delta_T \|_1 - \frac{1}{2} \| \Delta_T^\perp \|_1 , 
    \end{align*}
    where the last inequality uses Lemma \ref{lem:exist-cert-2}. 

    Now, by Lemma \ref{lem:prepare} and Lemma \ref{lem:infeas-2}, we have 
    \begin{align*}
        0 
        \ge 
        \frac{1}{2} \| \Delta_T^\perp \|_1 - \frac{1}{n^{20}} \| \Delta_T \|_1 
        \ge 
        \frac{1}{2} \| \Delta_T^\perp \|_1 - \frac{2}{n^{18}} \| \Delta_T^\perp \|_1 , 
    \end{align*}
    which implies $ \| \Delta_T^\perp \|_1 = 0 $. Finally another use of Lemma \ref{lem:infeas-2} implies $ \| \Delta \|_1 = 0 $, which concludes the proof. 
    
    % \< \sign(H),  P_{U} \Delta P_{U} \> + \< \sign (\Delta_{T}^\perp ) , \Delta_{T}^\perp \> 
\end{proof} 


% -----------------------------------

% Consider the random variable 
% \begin{align*} 
%     \( I - \P_{T_r} \) \P_i \P_{T_r} 
% \end{align*} 

% \begin{align*} 
%     \|  \| 
% \end{align*} 

% -----------------------------------


% Note that $ \E \[ \P_{T_r} \P_i \P_{T_r} \] = \P_{T_r} $, and by Lemma \ref{}, we have  
% \begin{align*} 
    % \left\| \E \[ \( \P_{T_r} \P_i \P_{T_r} - \P_{T_r} \)^p \] \right\|
    % \le 
    % 2^p 
% \end{align*} 

% Let $ H_r = Q \Lambda Q^\top $ be the eigenvalue decomposition of $H_r$. Since $U_r$ spans the column space of $H_r$, we have $ Q^\top U_r U_r^\top Q = I_r := \begin{cases} I_r & 0_{r \times (n-r)} \\ 0_{(n - r) \times r} & 0_{(n - r) \times (n-r)} . \end{cases} $



% % Since $ U_r $ spans the column space of $ H_r $, we know $ P_{U_r}  $ 
% % \begin{align*} 
% %     P_{U_r} 
% % \end{align*} 


% Now consider 
% \begin{align*}
%     & \; \P_{T_r} \P_i \P_{T_r} H 
%     = 
%     \P_{T_r} \( \u \u^\top U_rU_r^\top H \v \v^\top + \u \u^\top H U_rU_r^\top \v \v^\top - \u \u^\top U_rU_r^\top H U_rU_r^\top \v \v^\top \) \\ 
%     =& \; 
%     U_r U_r^\top \u \u^\top U_rU_r^\top H \v \v^\top +  \u \u^\top U_rU_r^\top H \v \v^\top U_r U_r^\top - U_r U_r^\top
%     \u \u^\top U_rU_r^\top H \v \v^\top U_r U_r^\top \\ 
%     & + 
%     U_r U_r^\top \u \u^\top H U_rU_r^\top \v \v^\top +  \u \u^\top H U_rU_r^\top \v \v^\top U_r U_r^\top + U_r U_r^\top \u \u^\top H U_rU_r^\top \v \v^\top U_r U_r^\top\\
%     &- 
%     U_r U_r^\top \u \u^\top U_rU_r^\top H U_rU_r^\top \v \v^\top - U_rU_r^\top \u \u^\top  H U_rU_r^\top \v \v^\top U_r U_r^\top + U_rU_r^\top \u \u^\top U_rU_r^\top H U_rU_r^\top \v \v^\top U_r U_r^\top . 
%     % =_d & \; 
%     % U_r U_r^\top \u \u^\top U_rU_r^\top H \v \v^\top +  \u \u^\top U_rU_r^\top H \v \v^\top U_r U_r^\top - U_r U_r^\top
%     % \u \u^\top U_rU_r^\top H \v \v^\top U_r U_r^\top \\ 
%     % & + 
%     % U_r U_r^\top \u \u^\top H U_rU_r^\top \v \v^\top +  \u \u^\top H U_rU_r^\top \v \v^\top U_r U_r^\top + U_r U_r^\top \u \u^\top H U_rU_r^\top \v \v^\top U_r U_r^\top\\
%     % &- 
%     % U_r U_r^\top \u \u^\top U_rU_r^\top H U_rU_r^\top \v \v^\top - U_rU_r^\top \u \u^\top  H U_rU_r^\top \v \v^\top U_r U_r^\top + U_rU_r^\top \u \u^\top U_rU_r^\top H U_rU_r^\top \v \v^\top U_r U_r^\top \\ 
% \end{align*}

% Since the distribution of $\v$ and $\u$ are rotation-invariant and reflection-invariant, we know that for any orthognal matrix $Q$, $ Q \v =_d \v $ and $ Q \u =_d \u $, where $=_d$ denotes distributional equivalence. This observation yields that 
% \begin{align*} 
%     & \; U_r U_r^\top \u \u^\top U_rU_r^\top H \v \v^\top
%     =_d 
%     U_r U_r^\top Q \u \u^\top Q^\top U_rU_r^\top Q \Lambda Q^\top \v \v^\top 
%     =_d
%     Q I_{:r} \u \u^\top I_{:r} \Lambda Q^\top \v \v^\top  . 
% \end{align*} 




